Computing Equilibrium in Matching Markets

Market equilibria of matching markets offer an intuitive and fair solution for matching problems without money with agents who have preferences over the items. Such a matching market can be viewed as a variation of Fisher market, albeit with rather peculiar preferences of agents. These preferences can be described by piece-wise linear concave (PLC) functions, which however, are not separable (due to each agent only asking for one item), are not monotone, and do not satisfy the gross substitute property-- increase in price of an item can result in increased demand for the item. Devanur and Kannan in FOCS 08 showed that market clearing prices can be found in polynomial time in markets with fixed number of items and general PLC preferences. They also consider Fischer markets with fixed number of agents (instead of fixed number of items), and give a polynomial time algorithm for this case if preferences are separable functions of the items, in addition to being PLC functions. Our main result is a polynomial time algorithm for finding market clearing prices in matching markets with fixed number of different agent preferences, despite that the utility corresponding to matching markets is not separable. We also give a simpler algorithm for the case of matching markets with fixed number of different items.

==> FixedAgentsIntroOld.tex <==

In this section, we study the problem of finding an exact equilibrium in the case where the number of agents $n$ is constant, and the number of different goods is an arbitrary number $m\in \mathbb{N}$.

For the algorithm in this section, we need to add a mild assumption that each agent has a unique most preferred item. More formally, for every agent $i\in [n]$, there is exactly one item $j$ such that $v_{ij}=\max_{z\in[m]}(v_{iz})$. The goal of this section is proving the following theorem by providing a polynomial time algorithm which finds the exact values of equilibrium prices and allocations.

\begin{theorem}\label{THM:FixedAgents}
Finding exact value of an equilibrium prices and allocations of a market with fixed number of agents in which agents have additive values, one unit of money, matching constraints and a unique most preferred item can be done in polynomial time.
\end{theorem}

We use theorem \ref{THM:CellDecomp} as the base of our algorithm. In order to do this, we have to characterize the equilibria with a set of polynomials using fixed number of variables. We wish to define a variable to represent the price of each item, however, since the number of items is not constant, this is not possible. Instead, for each agent, we define a variable which represents that agent's optimum utility in equilibrium. In section \ref{Sec:AgentsPriceBundleChar}, we show how these variables can be used to formulate the price of each item.

The next step in our algorithm is checking the market clearing conditions. Doing this in terms of variables and polynomials is not as straight forward: naively checking whether all the agents can get their 1 unit of items while their allocation is optimum, requires a non-constant ($\Omega(nm)$) number of variables that represent the agents' allocations in equilibria. Our main novel idea to get around this problem is showing that for every equilibrium pricing, there exists an allocation which can be described with $O(n^2)$ number of variables. This helps us check the market clearing conditions and find the equilibria by using theorem \ref{THM:CellDecomp}. All the missing proofs of section \ref{Sec:FixedAgents} are in appendix \ref{Sec:ApAgents}.

\textbf{General Outline and Techniques. }
In short, our algorithm searches the space of agents' optimal utilities and finds an equilibrium. For this, we need a tool for searching the space of agents' optimum utilities and a way to characterize of the equilibria of this market. For former, we use a cell decomposition technique which divides the space of agents' utilities into smaller pieces, called cells, each of which contains an set of values that share some properties. For latter we provide a bundling technique that helps us with characterizing the equilibria. In the rest of this section, we go into a more detailed description of these techniques which are the bases of our algorithm.

\textbf{Layered Cell Decomposition. } Our algorithm for fixed number of agents uses theorem \ref{THM:CellDecomp} as a tool for dividing the space of variables into cells and finding the equilibrium prices. A cell is a set values for the variables which make the defined polynomials have the same sign. Given a set of polynomials and variables, theorem \ref{THM:CellDecomp} iterates all the feasible cells and tells us what is the sign of each defined polynomial in each of these cells. The general idea is to have agents' optimum utilities and assignments be represented with a set of variables.

For using theorem \ref{THM:CellDecomp} and keeping the running time polynomial, we have to make sure that the number of variables we define is constant and the number of polynomials and the degree of the polynomials that we define is polynomial in the input size.

The way we use this theorem is by defining some layers, each of which consists of a set of variables and polynomials. We start by defining the first layer of variables (agents' optimum values in equilibrium) and polynomials. Then we use the information that each cell provides (by giving us the sign of the polynomials in the first layer) in order to define the variables and polynomials of the second layer, which divide each cell of the previous layer into smaller cells. We continue this process a few times until we pinpoint the cells which only contain equilibrium prices and sample from these cells to find an equilibrium.

\textbf{Cell. } We use brute-force twice to find an assignment of items to agents. The first brute-force is for fixing an item which is in one of the optimum bundles of each agent. The second brute-force is for finding the items that each pair of agents are sharing. We generalize the definition of cell so that it includes an outcome of an iteration of theorem \ref{THM:CellDecomp} and brute-forces, i.e. sign of each of the defined polynomials, a selection of each of our brute-forces. Our algorithms iterates all the feasible cells and finds the ones which contain equilibria.

\textbf{Bundles. } In equilibria each agent spend exactly one unit of money and gets exactly a total of one unit of items. This means that in equilibrium if an agent gets some amount an item whose unit price is less than one, she should also get some amount an item whose unit price is more than one. Using this fact, for simplifying our polynomials, we use a bundling technique, in which each bundle consists of at most two different types of items. We define each of these bundles so that they contain exactly a total of one unit of items and the total unit price of the bundle is exactly 1. This means that if a bundle has an item with price more than one, it should also contain an item with price less than one. Here, we give a description and prove some basic properties of this bundling. First, we show that the allocations of items to agents, can be rewritten as the allocation of bundles to agents, when the bundles are defined in a certain way.

\begin{lemma}\label{Lem:Bundling}
In an equilibrium pricing $P$ with equilibrium allocation $X$, there exists a bundling $B$ of items such that
\begin{itemize}
\item[a.] Each bundle $b$ consists of at most two items. Two items $j$ and $k$ are in a bundle $b=(j,k)$ if and only if $p_j<1<p_k$. One item $z$ forms a bundle $b=(z)$ if and only if $p_z=1$.
\item[b.] For each bundle $b=(j,k)$, there exists a unique $0< \alpha_b < 1$ such that $p_b=\alpha_b p_j + (1-\alpha_b) p_k =1$ (for bundles with one item $\alpha_b=1$). We call $p_b$ the price of bundle $b$.
\item[c.] For each agent $i$, optimum allocation of the items to agent $i$ can be rewritten as allocation of a subset of the bundles $B_i \subseteq B$ (called $i$'s optimum bundles) to $i$.
\end{itemize}
\end{lemma}

We can define $B_i$ to be the maximal subset of $B$ such that for each $b\in B_i$ value of $i$ for $b$ is maximum among all the bundles in $B$. This is why we call $B_i$ the \textit{optimal bundles} of agent $i$. A corollary of the above lemma is that each agent should have more utility for the bundles that she use over the bundles that she does not use. The following corollary formalizes this statement. Let $v_{ib}$ be the value of agent $i$ for bundle $b$. For each bundle $b=(z)$ with one item, $v_{ib}=v_{iz}$ and for each bundle $b=(j,k)$ with two items, $v_{ib}=v_{ib}=\alpha_b v_{ia} + \alpha_b v_{ib}$.

\begin{corollary}\label{Lem:Bundlingd}
For each bundle $b$ in agent $i$'s optimum bundles $B_i$, value of $i$ for the bundle is maximum among all the bundles, i.e. $\forall b \in B_i, \forall b'\in B, v_{ib}\geq v_{ib'}$.
Furthermore, utility of $i$ in the equilibrium is $v_{ib}$.
\end{corollary}

Another useful property of this way of bundling items is that if we have four items $j$, $j'$, $k$ and $k'$ such that $p_j,p_{j'}<1<p_k,p_{k'}$, and $(j,k)$ and $(j',k')$ are in the set of optimum bundles of an agent, then $(j,k')$ and $(j',k)$ are also in the set of her optimum bundles. The following lemma formalizes this property.

\begin{lemma}\label{Lem:Bundlinge}
If $b_1=(j,k)$ and $b_2=(j',k')$ are in optimum bundles of agent $i$ ($B_i$), such that $p_j,p_{j'}<1<p_k,p_{k'}$, then $b_3=(j,k')$ and $b_4=(j',k)$ are also in $B_i$.
\end{lemma}

%In our algorithm, beside using the previous techniques, we also use brute-force twice to find an assignment of items to agents. The first brute-force is for fixing an item which is in one of the optimum bundles of each agent. The second brute-force is for finding the items that each pair of agents are sharing. For the second brute-force, we prove that the number of these shared items is at most 5. Since, the number of agents is assumed to be constant, the running time of these brute-force sub-algorithms are polynomial ($O(m^n)$ for the first, and $O(m^{5n^2})$ for the second one).

%We also generalize the definition of cell so that it includes an outcome of an iteration of theorem \ref{THM:CellDecomp} and brute-forces, i.e. sign of each of the defined polynomials, a selection of each of our brute-forces. Our algorithms iterates all the feasible cells and finds the ones which contain equilibria.


==> Related.tex <==
\section{Related Work}

The problem of allocating items to unit demand agents without money has been
studied extensively in both Economics and Computer Science literature.  Perhaps
the most well known solution to this problem is the Random Serial Dictatorship
(RSD) mechanism which has received the most attention in recent years. \RSD{} is
strategyproof, ex-post Pareto-efficient, symmetric (envy-free), and easy to
implement \citep{AS98}. However it is not interim Pareto-efficient, not even
with ordinal preferences. An alternative solution called probabilistic serial
(PS) was proposed by \cite{BM01} which is both envy-free and efficient with
respect to ordinal preferences, but is not strategyproof. The PS mechanism is
however not Pareto-efficient with cardinal preferences. The mechanism based on
market equilibrium from equal income considered in the current paper, which has
been studied earlier also by \cite{HZ79}, is both envy-free and efficient
with respect to cardinal preferences, though not strategyproof. In fact,
\cite{Z90} shows that for $\NumAgents \ge 3$ agents there is no mechanism that
is strategyproof, Pareto-efficient, and symmetric (envy-free). We should also note
that \cite{HZ79} propose an exponential time algorithm for finding approximate
equilibrium, whereas the current paper proposes an exact algorithm for
computing equilibrium which runs in polynomial time when either the number of
agents or the number of items is constant. Most of the recent work on the
problem of assignment without money has been focused on analyzing the efficiency
of RSD and PS mechanism under cardinal and/or ordinal preferences, e.g.,
\cite{BCK11a,ASZ14}.

The main techniques used in the current paper are based on the cell
decomposition result of \cite{CellDecomp:98} which has also been used by
\cite{Devanur:2008} to derive a polynomial time algorithm for a related
computing market equilibrium computation problem. However we should emphasis
that the result/algorithm of the current paper cannot be reduced to/derived from
\cite{CellDecomp:98} because the utility function in the current paper are
satiable, where as \cite{CellDecomp:98} require PLC utility functions which
cannot model satiable utility functions by definition.

% \begin{itemize} 
% \item \cite{SV15} \todo{Pooya?}
% \item \cite{R65} his result requires joint convexity, ours does not.
% \end{itemize}
